Improving Dialogue Agents by Decomposing One Global Explicit Annotation with Local Implicit Multimodal Feedback

We describe an approach for aligning an LLM-based dialogue agent based on global (i.e., dialogue-level) rewards, while also taking into account naturally-occurring multimodal signals. At a high level, our approach (dubbed GELI) learns a local, turn-level reward model by decomposing the human-provided Global Explicit (GE) session-level reward, using Local Implicit (LI) multimodal reward signals to crossmodally shape the reward decomposition step. This decomposed reward model is then used as part of the standard RHLF pipeline improve an LLM-based dialog agent. We run quantitative and qualitative human studies to evaluate the performance of our GELI approach, and find that it shows consistent improvements across various conversational metrics compared to baseline methods.

==> 1_intro_old.tex <==
%motivation 
%more straight forward and crisp -- people might get lost -- what the task is until 3 paragraph when we talk about reward redistribution - should be in the title
%first two paragraph: most of these tasks conversational come from self-reported survey -- post study -- the challenge is how to use that global reward -- and redistributing that to every episode in that data -- 
%example domains pedagogical agents -- distracting, either use more examples -- are you building a pedagogical examples more examples if you want, for education for healthcare, most of these tasks and datasets are have self-report only one rating self reported rating of their experience -- up front -- how do we redistribute to every episode multi-turned -- self report surveys 

%follow up defined research problem in the beginning with our proposed solutino - access and leveraging multimodality 
%define explicit and local in the beginning -- define the problem statement/research questions - 
%1. PS: difficulty in in redistributing single annotation over the long horizon --
%RQ1: how do we even redistribute 
%RQ2: how to use implicit local rewards such as multimodal rewards in grounding the distribution 
%following paragraphs go deeper 
%first paragraph: first year masters they need to understand what problem it is -- very layman terms 
%2nd paragraph: more technical implicit local/explicit global 
%don't link to any applications -- long-horizon conversation as a general converation of any kind 
% in the related section: prior work on dataset from specific domains 
%giving examples of datasets -- in education, medicine, therapy domains -- mostly have single reward of their experience -- user's conversation expericence 
%figure space of the redistribution: instead of applications on the right 
%everyone in this community is aware of acquiring annotations -- assign those rewards -- make annotators annotate each conversation -- turn episodes -- instead -- how to do we automize a way for post interaction reward -- across the whole span of the conversation
%make adaptive LLMs 
%related works -- redistributing reward -- cases where researchers resources to gain turn by turn annotations of this data -- across all domains (education/call centers -- in the discussions -- )
%final paragraph: how this contribution we made in this paper can be appllied to all different domains of conversational domains  -- huge 
%RL: conversation -- section for language models - first work cite -- point that out that it has never been done for conversation 
% related redistribution -- where they're applied NOT IN CONVO -- ONLY IN SIMULATORS PHYSICS
%point out citations // 

%how much effort people spend  granular -- how they gain this how expenisve 
%" Our community spends... xyz" 
% highlight even when there are granular annotations -- not participants subjects response (it is 3rd party -- subject to individual biases and may be misaligned, noisy) 




Adapting agents (e.g. LLMs) to specific use cases enables agents to perform better in their respective domains. For instance, LLMs adapted to the education domain can serve as pedagogical agent to provide more timely feedback; LLMs adapted to become a better conversational partner can generate utterances that are more coherent and context aware. Characterizing many desired target domains are (1) the availability and importance of multimodal data, which offer crucial signals for the task at hand (e.g. student facial expressions determining engagement).s (2) Single reward for a long horizon and multi-turn task. The task consists of a long sequence of actions and outcomes are culminations of them, and it is ambiguous and difficult to rate the quality of an individual action. As a result, many important application areas rely on a post-survey or final outcomes, such as learning outcomes in the educational domain, success of medical procedures. 

%problem setting
Therefore, it is difficult to apply popular paradigms of aligning language models to human preferences or agents with desired behaviors as they rely heavily on manual immediate fine-grained annotations. Consequently, we propose utilizing the single annotation in the form of post-surveys or final outcomes as a \emph{\textbf{explicit global}} reward, which captures the notion of the quality of the entire sequence of actions. Furthermore, we incorporate the multimodal signals as a form of \emph{\textbf{ implicit local}} reward, as multimodal signals can provide local grounding signals on the quality of individual actions. 
% \input{latex/z92_fig_highlevel}

%solution
Our proposed approach, VFRRD (Visual Feeback + Random Return Decomposition) is a novel paradigm to train a reward function in reinforcement learning setting which utilizes only a single explicit global reward and implicit local multimodal signals to output scores an of a particular action that an agent has taken. We utilize the single explicit global reward to automatically redistribute rewards based on return decomposition. To assist with the redistribution, we utilize the local implicit multimodal signals as a proxy to reshape the individual rewards. Via utilizing both, we can alleviate the need and difficulties to capture intermediate, manual, fine-grained rewards and utilize the readily-available wealth of multimodal behavioral data. 

%conversation domain
\input{latex/z97_fig_rewards}
We utilize our proposed approach to improve and adapt the free-form multi-turn conversational capability of a language model. Inherently, conversations are long term where meaningful rapport are built over long interactions, and rewards at the single utterance level is limited evaluating the overall quality of the interaction. Furthermore, conversations are multimodal and the listener's behavioral reactions offer feedback on speaker's utterance. Multimodal data of conversations are plentiful, hence, we train the reward function in a purely offline manner. To the best of our knowledge, we offer the first to approach to utilize reward redistribution to improve the social dialogue of large language models, with a single manual annotation. To this end, we run quantiative and qualitiative human studies, where we find that our proposed approach outperforms other approaches by a signficant margin and improves the language model's ability across most metrics (specificity, emotional connection, social, positivity, reusability and many others).  


% rapport, overall perceived  overall 
% u cant really evaluate a single utterance unless you want really short dialogue.
% We offer a novel approach to utilize reward redistribution in the context of a language model in a conversational task.


% We run automatic and human annotations on dialogue generation, where we find that our approach improves the language model's ability to stay on context, and coherence, relevance and fluency. 

% \item We offer the first to approach to utilize reward redistribution in the context of a language model in a conversational task.
%     \item We use an offline dataset, which is plentiful, to train the reward function, which is then used to update the language model 
%     \item Our approach is especially useful in modelling conversations, as this alleviates the burden of fine-grained manual annotations, only requiring a single post conversation survey
%     \item We utilize visual data to ground the reward estimates to actual human implicit behavior 
%     \item crystal clear: no visual feedback needed for RLHF step



% , decomposes the single explicit global reward via return decomposition. 


% use a single reward to automatically redistribute rewards based on return decomposition \cite{arjona2019rudder}. The redistribution considers the entire conversation when decomposing the reward and takes into account long dialogue contexts as a prompt to the language model.


% This way we utilize plentiful behavioral feedback and only use a single expensive manually annotated reward.


% the global 

% notion of the 

% the long-horizon nature: interactions are often m

% (1) a wealth of multimodal data and a sparse (often single) annotations on the outcomes 

% many popular paradigms of aligning language models to human preferences or agents with desired behaviors relies heavily on manual fine-grained annotations. However, often human preferences or successes cannot often cannot be determined at a fine-grained level. In the real world, in many settings, outcomes are culminations of many actions, and it is ambiguous and difficult to rate the quality an individual action. Therefore, preferences or success can only be determined over the entire  interaction, trajectory and/or multiple turns. As a result, many important application areas rely on a post-survey or final outcomes, such as learning outcomes in the educational domain, success of medical procedures, overall conversation quality in dyadic interactions. Such annotation can be seen as an explicit global manual annotation, which globally encapsulates the quality of the trajectory of human or agent behavior. 




% (i.e. learning outcomes in the educational domain, success of medical procedures, overall conversation quality).


% In order to adapt the agent for these specific use cases, we must be able to utilize the single delayed long-horizon reward.  




% \begin{itemize}
%     \item Motivate why conversational LLMs are important -- social chat is important
%     \item alignment: helpful? often only looking at utterance level rewards but we need more 
%     \item explicit global feedback: overall quality of conversation, notions of long term horzion, alleviate expensive burden
%     \item implicit behavioral feedback: plentiful, (FIND what these means) 
%     \item we combine the best of both worlds: we redistribute global feedback but shape it with implicit behavioral feedback to get a strong reward function 
%     \item importantly we use an offline dataset 
%     \item then use this redistributed reward funcction to improve the language model 
    
%     \item We offer the first to approach to utilize reward redistribution in the context of a language model in a conversational task.
%     \item We use an offline dataset, which is plentiful, to train the reward function, which is then used to update the language model 
%     \item Our approach is especially useful in modelling conversations, as this alleviates the burden of fine-grained manual annotations, only requiring a single post conversation survey
%     \item We utilize visual data to ground the reward estimates to actual human implicit behavior 
%     \item crystal clear: no visual feedback needed for RLHF step

%     % \item We utilize visual data to ground the reward estimates to actual human implicit behavior
    
% \end{itemize}

% Reinforcement Learning with Human Feedback (RLHF) is the de facto approach to align human preferences for Large Language Models (LLMs). However, RLHF requires fine-grained annotations per generated utterance. This results in major challenges. Firstly, it is costly as it requires manual annotations at each time step. Secondly, it is hard for annotators to gauge whether this response was appropriate with respect to the entire conversation, as in conversation one cannot often gauge the quality of a specific utterance without taking out the context of the whole conversation. Thirdly, it is ambiguous to annotate for how long of a context the human annotator need to consider when annotating for these errors. 

% Current paradigms of RLHF requires an online environment in which humans are required to interact with the system live. Since multimodal data of humans talking to humans is plentiful, utilizing offline reinforcement learning (offline RL) is a natural fit for our setting. We leverage offline multimodal datasets to train a reward function to discern conversational quality. which is then used in an reinforcement learning set-up to improve the policy of the large language model. 

% Therefore, we propose a method to use a single reward to automatically redistribute rewards based on return decomposition \cite{arjona2019rudder}. The redistribution considers the entire conversation when decomposing the reward and takes into account long dialogue contexts as a prompt to the language model. Our method is an adaptation of the least squares-based return decomposition and random return decomposition \cite{efroni2021reinforcement, ren2021learning}. The fundamental concept involves training a regression model that breaks down the trajectory return into the cumulative sum of per-step rewards. Importantly, while training the regression model, we jointly predict the visual affective cues to make sure that the estimate of the reward is grounded well to human implicit feedback, which provides signals about the perceived quality of the conversation. 

% Our contributions are as follows. 

% \begin{itemize}
%     \item We offer the first to approach to utilize reward redistribution in the context of a language model in a conversational task.
%     \item We use an offline dataset, which is plentiful, to train the reward function, which is then used to update the language model 
%     \item Our approach is especially useful in modelling conversations, as this alleviates the burden of fine-grained manual annotations, only requiring a single post conversation survey
%     \item We utilize visual data to ground the reward estimates to actual human implicit behavior 

%     \item crystal clear: no visual feedback needed for RLHF step

%     % \item We utilize visual data to ground the reward estimates to actual human implicit behavior
    
% \end{itemize}
 

% To evaluate the effectiveness of our approach, we utilize our proposed redistributed return approach to improve the free-form multi-turn conversational capability of a language model. We run automatic and human annotations on dialogue generation, where we find that our approach improves the language model's ability to stay on context, and coherence, relevance and fluency. 


% \textcolor{blue}{although useful, hard to redistibute rewards, guided redistribution single reward  -> motivating this from the beginning -> does not contain rich human cues  }

==> 7_discussion.tex <==

\subsection{Future Work}
\begin{itemize}
    \item changing longformer to larger model
    \item usage of other modalities 
\end{itemize}


==> z90_iteractive.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[t]
% \centering
% \resizebox{0.9\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]

% \begin{tabular}{@{}lcccc@{}}
% \toprule
% Baselines            & Connection      & Positivity  & Social      & Inclination \\
%                      & \multicolumn{4}{c}{(/100\%) ↑}                             \\ \midrule
% LLAMA2               & \textbf{30}     & 32          & \textbf{29} & 29          \\
% LLAMA2 + GELI        & \textbf{32}     & \textbf{32} & \textbf{33} & \textbf{32} \\ \midrule
% \multicolumn{1}{c}{} & Interestingness & Reuse       & Specific    & Sensible    \\ \midrule
% \textbf{LLAMA2}      & 34              & \textbf{31} & \textbf{64} & 73          \\
% LLAMA2 + GELI        & \textbf{28}     & \textbf{34} & \textbf{74} & \textbf{66} \\ \bottomrule
% \end{tabular}



% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
Baselines            & Connection      & Positivity & Social     & Inclination \\
                     & \multicolumn{4}{c}{(/100\%) ↑}                           \\ \midrule
LLAMA2               & 15.0 ± 1.0      & 16.0 ± 2.0 & 14.5 ± 0.5 & 14.5 ± 0.5  \\
LLAMA2 + GELI        & 16.0 ± 4.0      & 16.0 ± 3.0 & 16.0 ± 5.0 & 16.5 ± 5.5  \\ \midrule
\multicolumn{1}{c}{} & Interestingness & Reuse      & Specific   & Sensible    \\ \midrule
LLAMA2               & 17.0 ± 4.0      & 15.5 ± 1.5 & 82.0 ± 7.0 & 86.5 ± 1.5  \\
LLAMA2 + GELI        & 14.0 ± 2.0      & 17.0 ± 5.0 & 87.0 ± 4.0 & 83.0 ± 1.0  \\ \bottomrule
\end{tabular}
}

\caption{Human evaluation on interactive chatbot experiment}
\label{tab:interactive}

\end{table}

==> z91_tab_bigrl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering
\resizebox{1\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{@{}lcccccccc|c@{}}
\toprule
CANDOR \cite{reece2023candor} &x
  Connection &
  Positivity &
  Social &
  Inclination &
  Interestingness &
  Reuse &
  Specific &
  Sensible &
  GELI Score \\
 &
  \multicolumn{8}{c|}{(/100\%) ↑} &
  ↑ \\ \midrule
Human &
  16.00 $\pm$ 2.83 &
  16.33 $\pm$ 4.03 &
  19.67 $\pm$ 1.89 &
  17.33 $\pm$ 6.65 &
  17.33 $\pm$ 6.55 &
  17.33 $\pm$ 3.09 &
  {\color[HTML]{34A853} \textbf{82.67 $\pm$ 7.93}} &
  \textbf{85.33 $\pm$ 4.5} &
   N/A \\
LLAMA2 &
  \textbf{30.67 $\pm$ 8.73} &
  26.67 $\pm$ 6.65 &
  \textbf{25.67 $\pm$ 8.38} &
  26.00 $\pm$ 5.66 &
  \textbf{24.33 $\pm$ 7.76} &
  28.0 $\pm$ 5.72 &
  \textbf{77.33 $\pm$ 6.18} &
  \textbf{80.33 $\pm$ 5.91} &
  0.4929 \\
LLAMA2 + GE: RRD &
  21.33 $\pm$ 6.80 &
  16.33 $\pm$ 1.70 &
  18.00 $\pm$ 2.16 &
  17.67 $\pm$ 1.25 &
  18.00 $\pm$ 2.83 &
  11.33 $\pm$ 4.03 &
  68.67 $\pm$ 6.34 &
  69.0 $\pm$ 5.1 &
  0.5072 \\
LLAMA2 + LI: LS (Language Sentiment) &
  20.67 $\pm$ 7.04 &
  21.00 $\pm$ 4.90 &
  21.00 $\pm$ 5.72 &
  18.33 $\pm$ 8.22 &
  23.00 $\pm$ 3.56 &
  22.0 $\pm$ 6.98 &
  \textbf{82.0 $\pm$ 3.74} &
  \textbf{89.67 $\pm$ 4.19} &
  0.4852 \\
LLAMA2 + LI: VA (Visual Affect) &
  22.67 $\pm$ 4.19 &
  25.33 $\pm$ 5.44 &
  \textbf{31.33 $\pm$ 0.47} &
  28.67 $\pm$ 3.4 &
  19.33 $\pm$ 3.68 &
  26.0 $\pm$ 0.82 &
  67.67 $\pm$ 4.71 &
  {\color[HTML]{34A853} \textbf{90.0 $\pm$ 2.16}} &
  0.4858 \\
LLAMA2 + GELI: RRD+VA  &
  {\color[HTML]{34A853} \textbf{39.67 $\pm$ 7.32}} &
  {\color[HTML]{34A853} \textbf{44.33 $\pm$ 12.23}} &
  {\color[HTML]{34A853} \textbf{35.33 $\pm$ 10.87}} &
  {\color[HTML]{34A853} \textbf{37.33 $\pm$ 6.85}} &
  {\color[HTML]{34A853} \textbf{38.0 $\pm$ 10.2}} &
  {\color[HTML]{34A853} \textbf{41.67 $\pm$ 7.04}} &
  \textbf{80.33 $\pm$ 4.5} &
  \textbf{80.67 $\pm$ 10.5} &
  {\color[HTML]{34A853} \textbf{0.5419}} \\ \bottomrule
\end{tabular}
}
\caption{Human evaluation results on 100 samples for 3 seeds for 8 preference metrics where mean and std. are reported. {\color[HTML]{34A853}\textbf{Green}} indicates best score, \textbf{Bold} indicates scores that fall in the confidence interval of the best performing score. GELI \emojijelly performs better on 6 out of 8 metrics (emotional connection, positivity, social understanding, inclination, interestingness, reuse) and comparably to the best performing model on the other 2 metrics: specific and sensible.}
\label{tab:human_eval}


\end{table*}



==> z92_fig_highlevel.tex <==
\begin{figure}[]
    \begin{center}
    \includegraphics[width=1.2\linewidth]{figs/highlevel.pdf}
    \caption{Single Feedback form Long Horizon and Multimodal Data is common for many important downstream applications for Human-AI collaboration}
    \vspace{-5mm}
    \label{fig:high}
    \end{center}
\end{figure}

==> z94_tab_generations.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
Dialogue History                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & VFRRD                                                                                                                                                                                                                                                                                                                                                                                                                                                & Human                                                                                                                                                    & RRD                                                         & VF                                                    & Language Response Sentiment                                                                                              & LLAMA2                                                                                                                             \\ \midrule
\begin{tabular}[c]{@{}l@{}}AI: What, what’s the name of it?\\ \\ User: Easy Breath of Fire.\\ \\ AI: I actually want to look into it, I’m not writing it down. Grand fire.\\ \\ User: No Breath of Fire.\\ \\ AI: Oh, breath of fire. I was thinking of Grand theft Auto’s like grandpa passed fire.\\ \\ User: Yeah. Uh One and two are on smes, but three and four are on PS one now they tried to make a comeback on PS two but it was by a completely different developers and they just made a hack job of it.\\ \\ AI: Mhm Oh man.\\ \\ User: It was really bad, but the first four all great. Especially the first three, the fourth one is still good with, and it’s like the longest, but it has a couple of little challenges on it, like these little puzzles that the other ones don’t have that are kind of annoying.\\ \\ AI: Yeah, mm that’s very interesting.\\ \\ User: But uh what was that?\end{tabular} & Oh, I see. Yeah, the first three breath of fire’s are definitely classics. The nostalgia is there. And the little puzzles, you know, they can be fun. But it’s also cool to see how the series evolved over time. I mean, the first one was so simple, but it had this charm to it. And then the second one, you know, it’s like they added more depth to the story and the characters, and it was just really cool to see how it all came together. & \multicolumn{1}{c}{How we doing on time? I’m only asking because I actually forgot to eat lunch. My apologies. Mhm. Oh I said how are we doing on time?} & \multicolumn{1}{c}{Totally, totally grand fire. 100\% sure.} & \multicolumn{1}{c}{*chuckles* I’m glad you think so!} & \multicolumn{1}{c}{I apologize, I did not catch the name of the game you were referring to. Could you please repeat it?} & \multicolumn{1}{c}{Oh, yeah, I see. So you’re saying that the third and fourth games in the series are better than the first two?} \\ \bottomrule
\end{tabular}
}


\caption{RL scores}
\label{tab:gen}
\end{table*}

==> z95_tab_rl.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table*}[t]

% \centering
% \resizebox{1\textwidth}{!}{
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{tabular}{@{}lccccccccc@{}}
% \toprule
% Baselines &
%   \multicolumn{1}{l}{Connection} &
%   \multicolumn{1}{l}{Positivity} &
%   \multicolumn{1}{l}{Social} &
%   \multicolumn{1}{l}{Inclination} &
%   \multicolumn{1}{l}{Interestingness} &
%   \multicolumn{1}{l}{Reuse} &
%   \multicolumn{1}{l}{Specific} &
%   \multicolumn{1}{l}{Sensible} &
%   VF+RRD Score \\ \midrule
%  &
%   \multicolumn{8}{c|}{(/100\%) ↑} &
%   ↑ \\ \midrule
% Human &
%   16.00 ± 2.83 &
%   16.33 ± 4.03 &
%   19.67 ± 1.89 &
%   17.33 ± 6.65 &
%   17.33 ± 6.55 &
%   17.33 ± 3.09 &
%   \textbf{82.67 ± 7.93} &
%   \multicolumn{1}{c|}{\textbf{85.33 ± 4.5}} &
%    \\
% LLAMA2 &
%   \textbf{30.67 ± 8.73} &
%   26.67 ± 6.65 &
%   \textbf{25.67 ± 8.38} &
%   26.00 ± 5.66 &
%   \textbf{24.33 ± 7.76} &
%   28.0 ± 5.72 &
%   \textbf{77.33 ± 6.18} &
%   \multicolumn{1}{c|}{\textbf{80.33 ± 5.91}} &
%   0.4929 \\
% LLAMA2 + GE &
%   21.33 ± 6.80 &
%   16.33 ± 1.70 &
%   18.00 ± 2.16 &
%   17.67 ± 1.25 &
%   18.00 ± 2.83 &
%   11.33 ± 4.03 &
%   68.67 ± 6.34 &
%   \multicolumn{1}{c|}{69.0 ± 5.1} &
%   0.5072 \\
% LLAMA2 + LI (Language Response) &
%   20.67 ± 7.04 &
%   21.00 ± 4.90 &
%   21.00 ± 5.72 &
%   18.33 ± 8.22 &
%   23.00 ± 3.56 &
%   22.0 ± 6.98 &
%   \textbf{82.0 ± 3.74} &
%   \multicolumn{1}{c|}{\textbf{89.67 ± 4.19}} &
%   0.4852 \\
% LLAMA2 + LI (Visual Response) &
%   22.67 ± 4.19 &
%   25.33 ± 5.44 &
%   \textbf{31.33 ± 0.47} &
%   28.67 ± 3.4 &
%   19.33 ± 3.68 &
%   26.0 ± 0.82 &
%   67.67 ± 4.71 &
%   \multicolumn{1}{c|}{\textbf{90.0 ± 2.16}} &
%   0.4858 \\
% LLAMA2 + GELI &
%   \textbf{39.67 ± 7.32} &
%   \textbf{44.33 ± 12.23} &
%   \textbf{35.33 ± 10.87} &
%   \textbf{37.33 ± 6.85} &
%   \textbf{38.0 ± 10.2} &
%   \textbf{41.67 ± 7.04} &
%   \textbf{80.33 ± 4.5} &
%   \multicolumn{1}{c|}{\textbf{80.67 ± 10.5}} &
%   \textbf{0.5419} \\ \bottomrule
% \end{tabular}
% }
% \caption{RL scores}
% \label{tab:reward}


% \end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lccccccccc@{}}
\toprule
Baselines &
  Connection &
  Positivity &
  Social &
  Inclination &
  Interestingness &
  Reuse &
  Specific &
  Sensible &
  GELI Score \\ \midrule
 &
  \multicolumn{8}{c|}{(/100%) ↑} &
  ↑ \\ \midrule
Human &
  16.00 ± 2.83 &
  16.33 ± 4.03 &
  19.67 ± 1.89 &
  17.33 ± 6.65 &
  17.33 ± 6.55 &
  17.33 ± 3.09 &
  \textbf{82.67 ± 7.93} &
  \multicolumn{1}{c|}{\textbf{85.33 ± 4.5}} &
   \\
LLAMA2 &
  \textbf{30.67 ± 8.73} &
  26.67 ± 6.65 &
  \textbf{25.67 ± 8.38} &
  26.00 ± 5.66 &
  \textbf{24.33 ± 7.76} &
  28.0 ± 5.72 &
  \textbf{77.33 ± 6.18} &
  \multicolumn{1}{c|}{\textbf{80.33 ± 5.91}} &
  0.4929 \\
LLAMA2 + GE &
  21.33 ± 6.80 &
  16.33 ± 1.70 &
  18.00 ± 2.16 &
  17.67 ± 1.25 &
  18.00 ± 2.83 &
  11.33 ± 4.03 &
  68.67 ± 6.34 &
  \multicolumn{1}{c|}{69.0 ± 5.1} &
  0.5072 \\
LLAMA2 + LI (Language Response) &
  20.67 ± 7.04 &
  21.00 ± 4.90 &
  21.00 ± 5.72 &
  18.33 ± 8.22 &
  23.00 ± 3.56 &
  22.0 ± 6.98 &
  \textbf{82.0 ± 3.74} &
  \multicolumn{1}{c|}{\textbf{89.67 ± 4.19}} &
  0.4852 \\
LLAMA2 + LI (Visual Response) &
  22.67 ± 4.19 &
  25.33 ± 5.44 &
  \textbf{31.33 ± 0.47} &
  28.67 ± 3.4 &
  19.33 ± 3.68 &
  26.0 ± 0.82 &
  67.67 ± 4.71 &
  \multicolumn{1}{c|}{\textbf{90.0 ± 2.16}} &
  0.4858 \\
LLAMA2 + GELI &
  \textbf{39.67 ± 7.32} &
  \textbf{44.33 ± 12.23} &
  \textbf{35.33 ± 10.87} &
  \textbf{37.33 ± 6.85} &
  \textbf{38.0 ± 10.2} &
  \textbf{41.67 ± 7.04} &
  \textbf{80.33 ± 4.5} &
  \multicolumn{1}{c|}{\textbf{80.67 ± 10.5}} &
  \textbf{0.5419} \\ \bottomrule
\end{tabular}
\end{table}

==> z99_mainfig.tex <==
\begin{figure*}[t]
    \begin{center}
    \vspace{-2mm}
    \makebox[0.99\textwidth][c]{\includegraphics[width=0.99\textwidth]{figs/main_fig.pdf}}
    \caption{Top: Previous Reinforcement Learning with Human Feedback approaches to align LLMs to human preference, requiring manual annotations at each utterance. Bottom: Our proposed approach of Reinforcement Learning with Redistributed Human Feedback. We use a single post-survey annotation to automatically redistribute rewards.}
    \label{fig:main}
    \end{center}
\end{figure*}
